A computational fluid dynamics model for the small-scale dynamics of wave, ice floe and interstitial grease ice interaction

The marginal ice zone is a highly dynamical region where sea ice and ocean waves interact. Large-scale sea ice models only compute domain-averaged responses. As the majority of the marginal ice zone consists of mobile ice floes surrounded by grease ice, finer-scale modelling is needed to resolve variations of its mechanical properties, wave-induced pressure gradients and drag forces acting on the ice floes. A novel computational fluid dynamics approach is presented, that considers the heterogeneous sea ice material composition and accounts for the wave-ice interaction dynamics. Results show, after comparing three realistic sea ice layouts with similar concentration and floe diameter, that the discrepancy between the domain-averaged temporal stress and strain rate evolutions increases for decreasing wave period. Furthermore, strain rate and viscosity are mostly affected by the variability of ice floe shape and diameter.

==> package_preamble.tex <==
% -----------------------------------------
% UK language and time format
% -----------------------------------------
\usepackage[UKenglish]{babel}
\usepackage[UKenglish]{isodate}

% -----------------------------------------
% Page manipulation
% -----------------------------------------
\usepackage{lscape}

% -----------------------------------------
% Text manipulation
% -----------------------------------------
\usepackage{lipsum} % to fill in with arbitrary text
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor} % Allows text to be written in different colours
\usepackage[final, babel, protrusion=true,expansion=true]{microtype}
\usepackage[super]{nth}
\usepackage{setspace}

% -----------------------------------------
% Mathematics packages
% -----------------------------------------
\usepackage[fleqn]{mathtools}
\usepackage{amsfonts,amssymb,amsthm,amsbsy}
\usepackage[binary-units=true]{siunitx}
\usepackage{wasysym} % diameter symbol

% -----------------------------------------
% Text fonts
% -----------------------------------------
%\usepackage[sc,osf]{mathpazo} % add possibly `sc` and `osf` options
%\usepackage{eulervm}
%\usepackage{mathptmx}
\usepackage{newtxtext}
\usepackage[varg, cmintegrals, cmbraces]{newtxmath} % has to be placed after amsmath
\usepackage{eufrak}
\usepackage{ulem}

% -----------------------------------------
% Pictures/Images packages/commands
% -----------------------------------------
% Obsolete: sufigure
% Buggy: subfig - Hyperref doesn't work properly 
%\usepackage[tight,footnotesize]{subfigure}
\usepackage{graphicx}
\usepackage{float}
\usepackage{fancybox}
% Draws a frame around picture
\usepackage[export]{adjustbox}
\usepackage[hypcap]{caption}
\usepackage{subcaption} 
\usepackage{epstopdf}

\usepackage{soul}
\newcommand{\hlc}[2][yellow]{ {\sethlcolor{#1} \hl{#2}} }

% -----------------------------------------
% Tables
% -----------------------------------------
\usepackage{booktabs}
\usepackage{multirow}

% -----------------------------------------
% Lists
% -----------------------------------------
\usepackage{enumitem}


% -----------------------------------------
% Bibliography related packages/commands
% -----------------------------------------
% Using the NATBIB referencing environment
%\usepackage[square,sort,numbers]{natbib}
%
% Using the BIBLATEX referencing environment
%\usepackage[backend=biber,natbib=true]{biblatex}
%\usepackage[natbib=true]{biblatex}
%\bibliography{./Reference/MyRef}
%
% Handle cross-referencing
\usepackage[colorlinks=true,allcolors={blue},bookmarks]{hyperref}
%
% Create web-link for every DOI 
%\usepackage{doi}

% -----------------------------------------
% Display algorithms
% -----------------------------------------
%\usepackage{algorithmic}
%\usepackage{algorithm}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother
%\newcommand{\INDSTATE}[1][1]{\STATE\hspace{#1\algorithmicindent}}


% -----------------------------------------
% Table manipulation
% -----------------------------------------
\usepackage{multirow}


% -----------------------------------------
% SI Units manipulation
% -----------------------------------------
\usepackage[binary-units=true]{siunitx}


% -----------------------------------------
% TOC related stuff
% -----------------------------------------
% Include Appendix in TOC
\usepackage[titletoc]{appendix}
\usepackage{accents}

% Extend the TOC numbering
\setcounter{secnumdepth}{4}
\setcounter{tocdepth}{4}


% -----------------------------------------
% Nomenclature related stuff
% -----------------------------------------
\usepackage{todonotes}
\usepackage[refeq,refpage]{nomencl}
% command : makeindex thesis.nlo -s nomencl.ist -o thesis.nls
% Line spacing in nomenclature
\setlength{\nomitemsep}{-\parsep}
% Defining section in nomenclature
%\renewcommand{\nomgroup}[1]{%
%\ifthenelse{\equal{#1}{A}}{\item[\textbf{\textit{Symbols}}]}{
%\vspace{0.1cm}
%\ifthenelse{\equal{#1}{B}}{\item[\textbf{\textit{Greek Letters}}]}{}
%\vspace{0.15cm}
%\ifthenelse{\equal{#1}{C}}{\item[\textbf{\textit{Acronyms}}]}{}}}


% -----------------------------------------
% Display line numbers
% -----------------------------------------
\usepackage[switch,right,displaymath,mathlines]{lineno}
%\linenumbers
